SecondPose: SE(3)-Consistent Dual-Stream Feature Fusion for Category-Level Pose Estimation

Category-level object pose estimation, aiming to predict the 6D pose and 3D size of objects from known categories, typically struggles with large intra-class shape variation. Existing works utilizing mean shapes often fall short of capturing this variation. To address this issue, we present SecondPose, a novel approach integrating object-specific geometric features with semantic category priors from DINOv2. Leveraging the advantage of DINOv2 in providing SE(3)-consistent semantic features, we hierarchically extract two types of SE(3)-invariant geometric features to further encapsulate local-to-global object-specific information. These geometric features are then point-aligned with DINOv2 features to establish a consistent object representation under SE(3) transformations, facilitating the mapping from camera space to the pre-defined canonical space, thus further enhancing pose estimation. Extensive experiments on NOCS-REAL275 demonstrate that SecondPose achieves a 12.4% leap forward over the state-of-the-art. Moreover, on a more complex dataset HouseCat6D which provides photometrically challenging objects, SecondPose still surpasses other competitors by a large margin.

==> sections/old/1intro.tex <==
\section{Introduction}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/Teaser.pdf}
    \caption{This is just a placeholder for the teaser. We need a teaser here, maybe the unified representation of the object in the feature space. You can visualize the features of dino alone, geometric features alone and fused dual-stream features.}
    \label{fig:teaser}
\vspace{-0.5cm}
\end{figure}

In recent years, object pose estimation has emerged as a crucial task in computer vision, finding applications in diverse fields such as augmented reality~\cite{marchand2015pose,tan20176d,Tjaden_2017_ICCV}, robotic manipulation~\cite{fang2020graspnet,sundermeyer2021contact,wang2021demograsp,zhai2022monograspnet,chen2023keypoint}, and medical applications~\cite{busam2015stereo,esposito2016multimodal,busam2018markerless}. The fundamental goal of object pose estimation is to predict the rotation and translation of an object in three-dimensional space based on its appearance in a two-dimensional RGB or RGBD image.

Many methods have been proposed to solve this task from various perspectives and have achieved outstanding results on public benchmarks~\cite{hinterstoisser2011multimodal,kaskman2019homebreweddb,calli2015benchmarking,xiang2018posecnn,wang2022phocal,jung2022housecat6d,sundermeyer2023bop}. Most of these methods focus on instance-level pose estimation, where each network is trained and tested on a single object instance~\cite{manhardt2019explaining,labbe2020cosypose,wang2021gdr,su2022zebrapose}.
Workflows typically integrate 2D-3D correspondences~\cite{wang2021gdr,gao2022polarimetric,su2022zebrapose} as key interim steps, succeeded by a refining stage~\cite{labbe2020cosypose,busam2020like,megapose}.
However, their generalization and scalability are limited, as the 3D object model is required, and an individual network needs to be trained for each instance.

Category-level pose estimation, in contrast, aims at scenarios involving unseen objects of a known category, where the objective is to generalize the pose estimation process across various instances within a semantic class.
Recent methods in the domain of category-level pose estimation~\cite{wang2019normalized,manhardt2020cpspp,lin2021dualposenet,chen2021fsnet,lin2023vinet} have specifically aimed at training on multiple objects within one category. These methods demonstrate the capability to generalize to unseen objects from the same category, enhancing the adaptability of the pose estimation field.

Some methods deploy RGB and depth information for this task~\cite{wang2019normalized,chen2021fsnet,di2022gpvpose,lin2023vinet}.
We study an input extension by pairing it with embeddings generated from a large vision transformer (ViT), namely DINOv2~\cite{oquab2023dinov2}. 
DINOv2 is a ViT foundation model that leverages self-supervision together with large scale data curation that helped surpassing similar models such as DINO~\cite{caron2021dinov1} and CLIP~\cite{radford2021clip}.
DINOv2 shows strong generalization capabilities for its embedding patch features that are proven to be useful to establish consistent matches across a wide variety of semantically similar image content.
Category level pose estimation needs exactly this to establish correspondences between semantically similar regions between instances of a given class.
To this end, we inject DINOv2 features as side-information into \OURS to provide additional visual cues for the model to help find correspondences within a category using RGBD input.

Historically, the field of RGBD-based pose estimation relied on handcrafted RGBD feature matching, specifically leveraging point pair features (PPF)~\cite{drostppf}. PPFs are established by pairwise comparison of object regions and their approximated normals from the depth map and provide a powerful rotation-invariant descriptor that facilitates correspondence matching between 3D CAD model and input depth map. Despite its competitiveness in this regard~\cite{sundermeyer2023bop}, a notable drawback of this approach lies in its inefficiency, primarily attributable to the expansive voting space involved when the entire image is used. This inefficiency has been effectively addressed by pre-filtering locations using learned instance segmentation techniques~\cite{konig2020hybridppf}. While we do not have access to a 3D model at test time, we still build on top of these findings and integrate into \OURS~pre-filtered PPFs from the input images as a strong rotation-invariant geometric cue.
To summarize, our main contributions are threefold:
\begin{enumerate}
    \item We propose the idea of \textbf{joining} additional visual cues from a \textbf{foundation model} together \textbf{with} geometric cues from a robust \textbf{3D descriptor} as complementary information to improve object pose estimation.
    \item We design \textbf{\OURS}, a \textbf{category-level RGBD pose estimation pipeline} that fuses visual features from \mbox{DINOv2} with the rotation-invariant geometric descriptions of PPF.
    \item Systematic \textbf{experimentation proves} that the additional \textbf{visuo-geometric} cues significantly \textbf{boost} pose prediction performance also under sever occlusion and clutter. \OURS~overcomes previous SotA methods that even use additional shape priors.
\end{enumerate}

==> sections/old/2rw.tex <==
\section{Related Works}
The pose estimation literature can be separated into methods that have access to object information during training, i.e. \textit{seen pose estimation}, and approaches that do not. Foundations models are currently mostly used to generalize the pose estimation task beyond the category domain.

\subsection{Seen Pose Estimation}
The traditional pursuit of \textit{instance-level} pose estimation involves establishing a consistent correspondence between an image and its associated 3D CAD model, defining a rigid transformation in space. Early data-driven efforts employed deep learning architectures for direct pose parameter regression~\cite{xiang2018posecnn,kehl2017ssd}. Modern RGB pipelines often integrate 2D-3D correspondences~\cite{wang2021gdr,gao2022polarimetric,su2022zebrapose} as intermediate steps. A typical pipeline starts with 2D object detection, then generates hypotheses that are subsequently refined~\cite{labbe2020cosypose,busam2020like,megapose}.
The challenge of \textit{visual ambiguities}~\cite{manhardt2019explaining,haugaard2022surfemb} arises due to one-to-many correspondences, leading to multiple equally valid poses.
%Addressing this, some approaches advocate predicting pose distributions instead of a single estimate\cite{murphy2021implicit,iversen2022ki,haugaard2023spyropose}.
In contrast to monocular RGB methods~\cite{xiang2018posecnn,zakharov2019dpod,wang2021gdr,su2022zebrapose}, former \textit{RGBD frameworks}~\cite{drostppf,hinterstoisser2011multimodal,he2020pvn3d,he2021ffb6d} leverage additional depth maps from commodity sensors. %Early works often utilized hand-crafted features~\cite{drostppf,hinterstoisser2011multimodal}. Deep learning pipelines either optimize separate feature extraction from RGB and depth channels~\cite{wang2019densefusion,he2020pvn3d,chen2020g2lnet} or use bidirectional fusion modules~\cite{he2021ffb6d} to combine color and distance information.
Building on previous concepts to learn embeddings for pose estimation~\cite{wohlhart2015learning}, OVE6D~\cite{cai2022ove6d} represents various 3D models in a feature space which can be used to condition a 6D pose pipeline.
%given an inference RGBD sample, and OVE6D factorizes object rotations into viewpoint and in-plane rotation components, facilitating accurate pose estimation with a 3D model rendered from various perspectives.

%A multitude of \textit{datasets}~\cite{hinterstoisser2011multimodal,brachmann2014,xiang2018posecnn,kaskman2019homebreweddb}, alongside established pipelines and synthetic network pretraining strategies~\cite{tremblay2018falling,denninger2020blenderproc}, and standardized evaluation protocols~\cite{sundermeyer2023bop}, collectively enable objective comparisons of pose estimation pipelines, advancing the field.
A multitude of \textit{datasets}~\cite{hinterstoisser2011multimodal,brachmann2014,xiang2018posecnn,kaskman2019homebreweddb} and standardized evaluation protocols~\cite{sundermeyer2023bop}, collectively enable objective comparisons of pose estimation pipelines, advancing the field.
However, scalability poses challenges for instance-based object pose estimation methods.
On one hand, meticulous annotation of high-quality 3D data is resource-intensive~\cite{Drost_2017_ICCV,laval_error,wang2022phocal,jung2023importance,jung2022housecat6d,gso}.
On the other hand, the conventional learning paradigm demands one network to be trained for each individual object.
Various strategies have emerged to address these challenges, including the use of synthetic data~\cite{denninger2020blenderproc}, weak labels~\cite{cai2020reconstruct,vutukur2022welsa,li2023nerf}, self-supervision~\cite{wang2020self6d,sock2020introducing,ruhkamp2023polarimetric}, and the incorporation of neural view-synthesis~\cite{yen2020inerf,chen2023texpose}.
However, the intrinsic scalability issue persists.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/Pipeline.pdf}
    \caption{This is just a placeholder for the pipeline. We need a pipeline here. We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.
    We need a pipeline here.}
    \label{fig:pipe}
\vspace{-0.2cm}
\end{figure*}

\subsection{Unseen Pose Estimation}
Initial strategies for learning monocular pose estimation for unseen objects employ techniques like 2D-3D feature-alignment~\cite{shugurov2022osop}, hypothesis scoring~\cite{okorn2021zephyr}, and render-and-compare refinement~\cite{megapose}. However, OSOP~\cite{shugurov2022osop}'s features lack rotation invariance, and the computational demands of ZePHyR~\cite{okorn2021zephyr} and MegaPose~\cite{megapose} remain high due to evaluating a large number of hypothesis samples.

Methods utilizing Point Pair Features (PPF)~\cite{drostppf} have long dominated the leaderboard for instance pose estimation~\cite{sundermeyer2023bop}. PPF relies on a handcrafted 3D descriptors that leverages pairwise distances and estimates and compares surface normals.
%While PPF does not demand training and enables pose estimation for unseen objects given a 3D CAD model, the quadratic growth of the voting space with considered points can lead to runtime bottlenecks. Combining PPF with learned 2D object segmentation from RGB~\cite{konig2020hybridppf} significantly accelerates this process.
PPFs extensive runtime requirement for feature voting has been accelerated by pairing it with a learned pre-filter stage~\cite{konig2020hybridppf}.
Although the initial PPF framerwork~\cite{drostppf} requires a 3D CAD model, we utilize PPF features in the absence of such as a complementary geometric cue for our model \OURS.
%Inspired by the rotation-invariant design of PPF, recent 3D point cloud matching pipelines for pure geometry matching~\cite{yu2022riga,wang2021you,yu2023roitr} incorporate its rotation-invariance overcoming the limitations of previous approaches~\cite{yu2021cofinet,huang2021predator,li2022lepard,Qin_2022_CVPR}.
Inspired by the rotation-invariant design of PPF, recent 3D point cloud matching pipelines for pure geometry matching~\cite{yu2022riga,wang2021you,yu2023roitr} incorporate this idea.
%A newer research line explores the incorporation of these geometry features for unseen pose estimation when a CAD model is provided. However, Zeropose~\cite{zeropose} and GCPose~\cite{gcpose} face challenges as their underlying 3D descriptor methods lack rotation invariance. Zeropose~\cite{zeropose} uses ImageBind~\cite{girdhar2023imagebind} and SAM~\cite{kirillov2023segment} foundation models to establish 3D-3D feature matching from GeoTransformer~\cite{Qin_2022_CVPR}. GCPose~\cite{gcpose} adopts the same descriptor principle~\cite{Qin_2022_CVPR}, complemented by explicit knowledge of object symmetries.
A very recent research line for object pose estimation explores the incorporation of these geometry features for unseen pose estimation when a CAD model is provided~\cite{zeropose,gcpose}. These methods, however, are limited by a 3D descriptors~\cite{Qin_2022_CVPR} that is not rotation-invariant.

Moving to the task of \textit{category-level pose estimation}, NOCS~\cite{wang2019normalized} establishes a normalized space for comparison objects of various scales, initiating research into supervised category-level methods~\cite{tian2020shape,chen2021fsnet,centersnap,di2022gpvpose}, as well as self-supervised refinement pipelines~\cite{manhardt2020cps++,lin2022selfdpdn}.
These approaches allow generalization to unseen objects of the same semantic class.
VI-Net~\cite{lin2023vinet} extends OVE6D~\cite{cai2022ove6d} in this regard thereby addressing the non-Euclidean nature of $\text{SO}\left(3\right)$~\cite{busam2017camera,zhou2019continuity}. Rotation prediction is factorized into a viewpoint rotation component and an in-plane rotation using spherical convolutions. The proposed approach in this paper builds on these advancements, leveraging the VI-Net backbone and targeting category-level pose estimation for unseen objects within a known semantic class.
%VI-Net~\cite{lin2023vinet} extends OVE6D~\cite{cai2022ove6d} in this regard thereby addressing the non-Euclidean nature of $\text{SO}\left(3\right)$~\cite{busam2017camera,zhou2019continuity}. Rotation prediction is factorized into a viewpoint rotation component, trained via binary classification, and in-plane rotation using spherical convolutions. The proposed approach in this paper builds on these advancements, leveraging the VI-Net backbone and targeting category-level pose estimation for unseen objects within a known semantic class.
\OURS~explores, however, how additionally injected visuo-geometric cues can enhance model performance by using PPF features together with the foundation model DINOv2~\cite{oquab2023dinov2}.

\subsection{Foundation Models and Generic Pipelines}
The aforementioned Zeropose~\cite{zeropose} uses ImageBind~\cite{girdhar2023imagebind} and SAM~\cite{kirillov2023segment} foundation models, but requires a 3D CAD model.
Other approaches investigate foundation models to generalize the pose estimation task further.

Concurrent to our work, scholars explore instance pose estimation from RGB and RGBD images, using reverse Structure from Motion (SfM) for \textit{generic pose estimation} where the task is to align a set of images to a query view of an object~\cite{liu2022gen6d,sun2022onepose,he2022oneposeplusplus}.
POPE~\cite{fan2023pope} extracts relative poses from a single input view, utilizing foundation models~\cite{kirillov2023segment,oquab2023dinov2}.
%POPE~\cite{fan2023pope} and NOPE~\cite{nguyen2023nope} extract relative poses from a single input view, utilizing foundation models~\cite{kirillov2023segment,oquab2023dinov2} and learned feature embeddings~\cite{nguyen2023nope} for probabilistic pose alignment.
Goodwin \etal~\cite{goodwin2022,goodwin2023you} elegantly extend a correspondence pipeline to object categories proposing a design that does not require retraining for emerging categories.
They leverage the foundational model features of DINO~\cite{caron2021dinov1} to establish correspondences between various object instances of a given semantic class where one reference RGBD view is matches to a target RGBD sequence of the same class.
%Matches between support view and target views are lifted with the depth map to 3D where pose estimation is facilitated using the Umeyama algorithm~\cite{umeyama1991least}.
While undoubtedly aiding rough object pose alignment, the absence of explicit object category training hinders their practical application until now.
The use of foundation models, however is shared.
We utilize DINOv2~\cite{oquab2023dinov2} embeddings as additional semantic input cues to visually guide \OURS~towards more accurate predictions.



==> sections/old/3method.tex <==
\section{Method}
We aim at handling the problem of category-level 9DoF object pose estimation from a single RGB-D image.
In particular, given an RGB-D image capturing the target object from a set of known categories, our goal is to recover its full 9DoF object poses, including $\boldsymbol{R} \in S O(3)$ and a $3 \mathrm{D}$ translation $t \in \mathbb{R}^3$ and a 3D metric size $s \in \mathbb{R}^3$. 

\iffalse
We tackle the problem of 3D pose estimation from an RGB-D object, which is to learn the transformation from the object canonical coordinate system to the camera observation system, represented by a $\boldsymbol{R} \in S O(3)$ and a $3 \mathrm{D}$ translation $t \in \mathbb{R}^3$ and a 3D size $s \in \mathbb{R}^3$. 
\fi

\subsection{Overview.}
As illustrated in Fig.~2, ROSE-Pose mainly consists of 3 subsequent modules to predict object pose from a single RGB-D input, \textit{i.e.} i) respective geometric and semantic feature embedding, ii) dual-stream feature fusion for the rotation-invariant object representation, iii) pose regression from the extracted representation via a pose estimator.

\textbf{Respective Feature Extraction.}
Geometric features Fg (Fig.~2 c) and semantic features Fs (Fig.~2 d) are extracted and resized to align the corresponding pixels.
Then backproject to the 3D space to get a point cloud.

\textbf{Dual-Stream Feature Fusion.}
Due to our rotation-invariant design and our observation that DINO-V2 features are approximately rotation-invariant, so directly concatenating them together yields a rotation-invariant object representation. 
We prove that such simple fusion method is powerful.

\textbf{Pose Regression.}
The representation Fr (Fig2 e) encapsulates pose information and can be directly used as input to any off-the-shelf pose estimator~\cite{di2022gpvpose, lin2023vinet}.

\textcolor{red}{after drawing the pipeline, this subsection should be refined accordingly.}

\iffalse
Following \cite{lin2023vinet}, we resort to a lightweight PointNet++ for translation and size estimation. Given an RGB-D 
image, we first segment the object of interest with Mask-RCNN \cite{he2017mask} following \cite{di2022gpvpose, lin2023vinet}. N points are randomly selected from the back-projected 3D point clouds $\boldsymbol{P} \in \mathbb{R}^{n \times 3}$ and input to the translation and size estimator.
Our method thus focus on the more challenging task of rotation estimation. \\
The RGB images are input to an pre-trained Vision Transformer\cite{oquab2023dinov2} to extract semantic-sensitive features $\boldsymbol{F_s} \in \mathbb{R}^{n \times c_s}$, and then rotation invariant geometric embedding $\boldsymbol{F_g} \in \mathbb{R}^{n \times c_g}$ are calculated from the 3D point clouds. The rgb values $\boldsymbol{C} \in \mathbb{R}^{n \times 3}$, 3D point clouds $\boldsymbol{P}$, geometric features $\boldsymbol{F_g}$ and semantic features $\boldsymbol{F_s}$ are input to our backbone jointly for rotation estimation.
\fi

\subsection{Hierarchical-panel Geometric Stream}
Our geometric embedding in this stream is based on the calculation of pair-wise $SE(3)$ equivariant Point Pair Features (PPF)~\cite{drostppf}. 
%We construct our pose-invariant coordinate representation by aggregating the PPF between the point of interest and neighborhood points in the multiple panels centered on it. We hierarchically concatenate the corresponding pose-invariant coordinate representations in each panel to enrich the representation power of our geometric features. (maybe can put in the intro)

\paragraph{Point Pair Features}Given a point cloud object denoted as $\boldsymbol{P}$, we consider each pair of points $(p_i, p_j)$ where $p_i, p_j \in \boldsymbol{P}$. Associated with each point, local normal vectors at $p_i$ and $p_j$ are represented as $\boldsymbol{n_i}$ and $\boldsymbol{n_j}$, respectively. The pairwise feature between points $p_i$ and $p_j$ can be formalized as:

\begin{equation}
f_{i,j} = [d_{i,j}, \alpha_{i,j}, \beta_{i,j}, \theta_{i,j}],
\end{equation}
where $d_{i,j} = \lVert p_j - p_i \rVert$ quantifies the Euclidean distance between points $p_i$ and $p_j$. $\alpha_{i,j} = \angle (\boldsymbol{n_i}, p_j-p_i)$ represents the angular deviation between the normal vector $\boldsymbol{n_i}$ at point $p_i$ and the vector extending from $p_i$ to $p_j$. $\beta_{i,j} = \angle (\boldsymbol{n_j}, p_j-p_i)$ signifies the angle subtended by the normal vector $\boldsymbol{n_j}$ at point $p_j$ with the aforementioned vector from $p_i$ to $p_j$. $\theta_{i,j} = \angle (\boldsymbol{n_j}, \boldsymbol{n_i})$ delineates the angular disparity between the normal vectors $\boldsymbol{n_j}$ and $\boldsymbol{n_i}$ at points $p_j$ and $p_i$, respectively.
As it eliminates the influence brought by the global coordinate, this descriptor becomes $SE(3)$ equivariant.

\paragraph{Geometric Feature Panel}
Based on the PPF, we propose a panel-based PPF to construct our geometric representation, which dilates the perception field while maintaining the merit of . For each point $p_i$ in the point cloud $\boldsymbol{P}$, there is a support panel $\mathcal{S}^i \subseteq \boldsymbol{P}$ whose cardinality $s_i = |\mathcal{S}^i|$. For all points $p_j \in \mathcal{S}^i$, we calculate the PPF $f_{i, j}$ between $p_i, p_j$ and the local coordinate representation $f^i_l$ of $p_i$ is further calculated by taking average:
\begin{equation}
f^i_l = \frac{1}{s_i}(\sum_j{d_{i,j}}, \sum_j{\alpha_{i,j}}, \sum_j{\beta_{i,j}},\sum_j{\theta_{i,j}})
\end{equation}


\begin{figure}[t]
  \centering
  
   \includegraphics[width=0.75\linewidth]{figures/methods/hierarchicalppf.pdf}
   \caption{\textbf{Hierarchical panel-based geometric features.} Inner panel contains points that are close to the point of interest, and outer panels contain points far from the point of interest.
   }
   \label{fig:onecol}
\end{figure}

\paragraph{From Single to Hierarchical Panels}
Even the mean aggregation in the panel can take the neighbor points into account. The inherent local representation limits its representation power, as the features brought by normals $\boldsymbol{n_i},\boldsymbol{n_j}$ are noisy when constraining the perception field. Inspired by CNN architecture, in which the features are extracted from local to global hierarchically, to make our geometric features more powerful, we sample multiple panels hierarchically from local to global.
Specifically, for integers $(k_0, k_1, k_2,..., k_l),\space 0 = k_0<k_1<k_2<...<k_l=|\boldsymbol{P}|-1$,  for each point $p_i\in \boldsymbol{P}$ we first rank its distance to any other points in $\boldsymbol{P}$ from smallest to largest:
\begin{equation}
    r_{i,j} = sort(d_{i,j})
\end{equation}
and construct support panels:
\begin{equation}
  \mathcal{S}^{i,m}  = \{p_j \in \boldsymbol{P}| k_{m-1}< r_{i,j}\leq  k_m \}, 1 \leq m \leq l,
\end{equation}
where $l$ is the number of panels. we then calculate the corresponding pose-invariant coordinate representations $f^{i,m}$ for each panel $\mathcal{S}^{i,m}$ and concatenate them to get the point-wise geometric features:
\begin{equation}
    f_{g}^i = [f^{i,1}_l,f^{i,2}_l, ... f^{i,l}_l ]
\end{equation}
with smaller $k$, the support panel is composed of points that are closer to the point of interest, while with larger k, the support panel is composed of points that are farther from the point of interest. By concatenating features calculated by panels of different scales, we combine geometric features in a way that balances details of local geometric landscapes and global instance-wise shape information. We show in the Sec.~\ref{exper} that such a design brings better performance than the single-panel one.

\textcolor{red}{explain why we need local to global geometric feature. DINO feature, we use deeper layer, contains more global information, we use local geometric feature to enhance the locality.}

\subsection{Semantic-aware Features by Pre-trained Vision Transformer}
We use DinoV2\cite{oquab2023dinov2} as our semantic-aware feature extractor. As \cite{zhang2023tale} shows, DinoV2 can extract semantic-aware information from RGB images that is helpful is zero-shot semantic correspondence matching, which indicates that it contains rich semantic information. In pose estimation tasks, such extra information can give salient boost of performance. In the other hand, DinoV2 features also contains global instance-wise information, such as category and pose of the instance. 

\textbf{DinoV2 Features of Higher Layer with Global Information}
We use the "token" facet from the last last layer (11 th.) as our extracted semantic feature, as according to \cite{zhang2023tale}, the features of deeper layers exhibits the best semantic matching performance, which means it shows best consistency regarding semantic correspondence across different objects.  The feature from deeper layer also contains more global semantic information. 

\textbf{DinoV2 Feature as Quasi Pose-invariant Semantic Feature}
\cite{zhang2023tale} also shows that DinoV2 features perform well when matching keypoints of the same object of different poses, which means the semantic information extracted is quasi pose-invariant.

\textbf{Down-sampling of DinoV2 Feature for Computational efficiency}
For computational efficiency we down-sample the DinoV2 features to resolution of $15\times 15$. Our experiments shows that even with such low resolution, our pose estimation results is significantly 
boosted. 
\subsection{Fusing Multiple Streams of Features}
Our backbone model\cite{lin2023vinet} is based on spherical feature map and ResNet\cite{he2016deep}. It first scatters the 3D point coordinate to a spherical surface, and fill the feature map with each point's corespondent features respectively.  A natural way of fusing different streams of features is thus creating individual spherical feature map and having individual ResNets for each feature stream, concatenate their features at each stage of the ResNets and input to another ResNet decoder in a U-net manner. The bottle-neck layer insures that the final feature map contains high-level global information, while the decoder fusing features from earlier layers from ResNets of each feature streams preserves the local details. The output of the decoder is used to estimate the rotation.

\textbf{Pose-invariant features boosts performance}
The task of rotation estimation can be compared to a more difficult task of predicting each point's 3D coordinate in canonical space, which is pose-invariant.
Our experiments show that rotation invariant features boosts performance of this task. With known 3D coordinate in canonical space, the rotation estimation becomes trivial.\\
An easier task would be predicting for each point in the point cloud the corresponding point on the shape-prior, which is also pose-invariant. Prior-based methods have shown knowing correspondence of points on shape priors and points in point clouds benefits rotation estimation. \\
We believe there is a deep link between the aforementioned two tasks and the task of rotation estimation. Both of the two tasks outputs a pose-invariant feature of the point cloud, which makes rotation estimation easier. Our designed pose-invariant semantic feature and geometric feature serves the same purpose.

\textcolor{red}{why we fuse them in a rotation-invariant manner? directly fusing them with point cloud features have some drawbacks? DINO is approximately rotation-invariant, constructing a space that is approximately linear to the human-defined canonical space.}


 



==> sections/old/5conc.tex <==
\section{Conclusion}

\textbf{Limitations.}
